Interactive Segmentation Model for Placenta Segmentation from 3D Ultrasound images

Placenta volume measurement from 3D ultrasound images is critical for predicting pregnancy outcomes, and manual annotation is the gold standard. However, such manual annotation is expensive and time-consuming. Automated segmentation algorithms can often successfully segment the placenta, but these methods may not consistently produce robust segmentations suitable for practical use. Recently, inspired by the Segment Anything Model (SAM), deep learning-based interactive segmentation models have been widely applied in the medical imaging domain. These models produce a segmentation from visual prompts provided to indicate the target region, which may offer a feasible solution for practical use. However, none of these models are specifically designed for interactively segmenting 3D ultrasound images, which remain challenging due to the inherent noise of this modality. In this paper, we evaluate publicly available state-of-the-art 3D interactive segmentation models in contrast to a human-in-the-loop approach for the placenta segmentation task. The Dice score, normalized surface Dice, averaged symmetric surface distance, and 95-percent Hausdorff distance are used as evaluation metrics. We consider a Dice score of 0.95 a successful segmentation. Our results indicate that the human-in-the-loop segmentation model reaches this standard. Moreover, we assess the efficiency of the human-in-the-loop model as a function of the amount of prompts. Our results demonstrate that the human-in-the-loop model is both effective and efficient for interactive placenta segmentation. The code is available at \url{https://github.com/MedICL-VU/PRISM-placenta}.

==> table/backup.tex <==
\begin{table*}[t]
\caption{Quantitative results. Bold  indicates best performance.  PRISM-plain is a simplified model for a fair comparison to methods not allowing BB prompts \cite{gong20233dsam,li2023promise,wang2023sam}, and methods\cite{kirillov2023segment,gong20233dsam,li2023promise,wang2023sam} only using 1 point prompt per input. For liver tumor, 10 points are used for all methods to accommodate multiple tumors.} 

\label{main_table}
\small
\begin{center}
    \begin{tabular}{ l  | c |c |c }
    
    \hline
    \multicolumn{1}{l}{Methods} &   \multicolumn{1}{c}{Anterior (n=14)} & \multicolumn{1}{c}{Posterior (n=10)} & \multicolumn{1}{c}{Overall (n=24) change n to another place}\\
    \hline
    % nnU-Net \cite{isensee2021nnu} &    43.91 / 52.52 & 41.65 / 62.54 & 60.10 / 75.41 \\
    Automatic \cite{schwartz2022fully} &    90.46 / 80.72 & 89.42 / 75.75 & 90.03 / 78.65 \\
    
    SAM \cite{kirillov2023segment} &    &  &  \\ 

    % SAM-Med2D \cite{cheng2023sam} &     &   &   &   \\

    3DSAM-adapter \cite{gong20233dsam} &   &  &  \\

    
    ProMISe \cite{li2023promise} &    &  &   \\

    SAM-Med3D \cite{wang2023sam} &    &   & 57.02 / 24.71  \\

    % SAM-Med3D-organ &   70.75 / 91.03  & 76.40 / 97.75  &  66.52 / 77.97  & 88.20 / 97.80 \\
    % SAM-Med3D-turbo &   73.77 / 94.95  & 74.87 / 96.43  & 69.36 / 81.70 &  89.26 / 98.40 \\



    
    PRISM-plain &  87.04 / 72.43   &  88.55 / 73.40 &  87.66 / 72.83  \\


    PRISM-plain with box &  87.44 / 73.96   &  87.76 / 70.96 &  87.58 / 72.71  \\


    PRISM-plain 10 points with box &  89.31 / 78.48   &  89.20 / 75.74 &  89.26 / 77.34  \\


    PRISM-ultra (centerline random) &  97.35 / 99.68  &  97.01 / 99.44  & 97.15 / 99.54 \\

    PRISM-ultra (centerline) &   97.41 / 99.75  &  97.31 / 99.70  & 97.55 / 99.82 \\


    PRISM-ultra (contour random) &  96.88 / 99.47  &  97.29 / 99.77  & 97.04 / 99.59 \\

    PRISM-ultra (contour) &  96.05 / 98.85  & 96.48 / 99.21 & 96.22 / 99.00 \\


    PRISM sagittal 1 point &  86.06 / 70.68  &  83.50 / 63.28 &  85.01 / 67.59  \\

    PRISM sagittal 1 point with box &  86.06 / 71.25  &  82.83 / 63.54 &  84.72 / 68.03  \\
    
    PRISM sagittal 10 point with box &  88.16 / 74.89  &  86.52 / 68.99 &  87.47 / 72.43  \\
        
    PRISM-ultra sagittal (centerline random) &  96.24 / 98.85  & 96.64 / 99.25 & 96.41 / 99.02 \\

    PRISM-ultra sagittal (centerline) &  96.33 / 99.01  & 96.87 / 99.58 & 96.56 / 99.25 \\


    PRISM-ultra sagittal (contour random) &  96.18 / 99.16  & 96.54 / 99.40 & 96.33 / 99.26 \\

    PRISM-ultra sagittal (contour) &  95.51 / 97.95  & 96.10 / 98.98 & 95.75 / 98.38 \\
    \hline     

     
\end{tabular} 

\end{center}
\end{table*}





==> text/introduction_old.tex <==
\clearpage

\section{Introduction}
Placenta volume measurement from 2D and 3D ultrasound (US) images is important for predicting birthweight \cite{schwartz2012two}, stillbirth \cite{seaton2012socioeconomic} and adverse pregnancy outcomes, such as preeclampsia \cite{redman2005latest,schwartz2014first} and intrauterine growth restriction \cite{biswas2008gross}, which contribute significantly to perinatal morbidity and mortality.


Human annotations of the placenta are considered the gold standard in clinical settings to ensure precise measurements. However, obtaining annotations is time-consuming, expensive, and requires expert knowledge. In contrast, an early study has first developed a fully automatic algorithm using multi-atlas segmentation techniques to successfully segment the placenta \cite{oguz2016automated}. In recent years, deep learning-based automatic approaches have demonstrated state-of-the-art performance as the leading method for placenta segmentation \cite{looney2018fully,looney2021fully,looney2017automatic,oguz2018combining,pouch2020automated,schwartz2022fully,zimmer2023placenta}.



Despite their advancements, these automatic segmentation methods do not consistently deliver high performance in every case. Robust segmentation of the placenta remains challenging due to unclear boundaries in US images \cite{wang2021deep}, especially during early pregnancy when the placenta and uterine tissue are less distinct. This issue is further complicated by the weak contrast and inherent noise in 3D US images, which obstruct the accurate delineation of placental boundaries. Additionally, robust placental segmentation needs to be considered for individual anatomical variations \cite{fiorentino2023review}, and it is influenced by uterine contractions that can dramatically alter the shape of the placenta. The segmentation quality is also affected by the location of the placenta, and a posterior position brings additional challenges due to the shadow effects \cite{xu2021shadow} and attenuation artifacts commonly seen in US imaging. More importantly, these data-driven methods require a substantial amount of training data to cover all such variations to achieve superior performance \cite{wang2023ssl2,luo2021semi}, which is a well-known challenge in the medical domain where data is often limited. Thus, developing a generalized method that can accurately segment the placenta in such challenging conditions without extensive user intervention is crucial for integrating placental morphometry into routine clinical practice.


An interactive segmentation method could serve as a potential alternative for addressing variabilities and improving the robustness of placenta segmentation. A previous study has \cite{oguz2020minimally} demonstrated that a semi-automatic approach with input achieves consistent performance between anterior and posterior placentas during the early stages of pregnancy, even with significant variations. However, its accuracy may not meet the requirements for routine clinical use.


The deep learning-based interactive segmentation method, Segment Anything Model (SAM) \cite{Kirillov_2023_ICCV}, has demonstrated its generalizability and ability to produce precise segmentation and has been widely adopted in the medical domain \cite{ma2024segment,li2023promise,gong20233dsam,wang2023sam,cheng2023sam,li2024prism}, including for the US applications \cite{yao2023false,lin2023samus,tu2024ultrasound}. These SAM-based models require users to provide prompts, such as points \cite{li2023promise,gong20233dsam,wang2023sam,cheng2023sam,li2024prism,tu2024ultrasound,lin2023samus}, boxes \cite{yao2023false,ma2024segment,li2024prism}, scribbles \cite{li2024prism}, and masks \cite{wang2023sam,cheng2023sam,li2024prism}, for interactions. Unfortunately, even with such interactions, these current studies designed for US applications do not consistently produce robust segmentation for clinical use. To achieve robust segmentation, some of these methods \cite{wang2023sam,cheng2023sam,li2024prism} are designed as human-in-the-loop, and the PRISM \cite{li2024prism} stands out as it achieves human-level performance, making it an effective interactive segmentation model suitable for clinical routine. Unlike other methods that accept limited types of visual prompts for interaction, PRISM accommodates all types of visual prompts to achieve precise segmentation. The iterative design and flexible prompts allow the users to refine the segmentation until it meets their expectations. However, it was not originally designed for ultrasound imaging applications and its performance is unknown.





In this paper, we evaluate the previously proposed PRISM for placenta segmentation from US images. I will write this based on the results.

 






\clearpage
